SPARS3R: Semantic Prior Alignment and Regularization for Sparse 3D Reconstruction

Recent efforts in Gaussian-Splat-based Novel View Synthesis can achieve photorealistic rendering; however, such capability is limited in sparse-view scenarios due to sparse initialization and over-fitting floaters. Recent progress in depth estimation and alignment can provide dense point cloud with few views; however, the resulting pose accuracy is suboptimal. In this work, we present SPARS3R, which combines the advantages of accurate pose estimation from Structure-from-Motion and dense point cloud from depth estimation. To this end, SPARS3R first performs a Global Fusion Alignment process that maps a prior dense point cloud to a sparse point cloud from Structure-from-Motion based on triangulated correspondences. RANSAC is applied during this process to distinguish inliers and outliers. SPARS3R then performs a second, Semantic Outlier Alignment step, which extracts semantically coherent regions around the outliers and performs local alignment in these regions. Along with several improvements in the evaluation process, we demonstrate that SPARS3R can achieve photorealistic rendering with sparse images and significantly outperforms existing approaches.

==> figures/3d_point/3dpoint_align.tex <==

\definecolor{SfM}{RGB}{100 , 156, 64}
\definecolor{Mast3r}{RGB}{4,36,51}
\begin{figure}[h!]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/3d_point/global_align.png}  % Replace with your image path
        \caption{Global Aligner}
        \label{fig:subfig1}
    \end{subfigure}
    \hfill
    % Second subfigure
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/3d_point/semantic_align.png}  % Replace with your image path
        \caption{Semantic Aligner}
        \label{fig:subfig2}
    \end{subfigure}
    % Main caption
    \caption{Comparison of 3D points with different alignment methods from an aerial view. The bounding boxes highlight the 3D points of the building using \textcolor{SfM}{SfM} and \textcolor{Mast3r}{Mast3r}.}
    \label{fig:main_figure}
\end{figure}

==> figures/depth_comp.tex <==
\renewcommand\thesubfigure{\roman{subfigure}}

\begin{figure}[!htb]
    \centering
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[b]{ccc}
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/depths/_DSC8680_mast3r.png}
            \caption{aa}
            \label{img:rgbd_deform}
        \end{subfigure} &

        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/depths/_DSC8680_marigold.png}
            \caption{marigold}
            \label{img:defocus}
        \end{subfigure} \\
        
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/depths/DSCF0762_mast3r.png}
            \caption{}
            \label{img:kernel_size}
        \end{subfigure} &
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/depths/DSCF0762_marigold.png}
            \caption{}
            \label{img:speed}
        \end{subfigure} 

    \end{tabular}
    \caption{hahaha }
    \label{fig:depth_comp}

% \vspace{-1.5em}
\end{figure}

==> figures/poses/pose.tex <==
\begin{figure}[h!]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Poses/Bicycle_pose_vis_fig.png}  % Replace with your image path
        \caption{Bicycle}
        \label{fig:subfig1}
    \end{subfigure}
    \hfill
    % Second subfigure
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Poses/bonsai_pose_vis_fig.png}  % Replace with your image path
        \caption{Bonsai}
        \label{fig:subfig2}
    \end{subfigure}
    % Main caption
    \caption{The comparison of camera poses of training views . We regard the dense view pose generated by COLMAP as ground truth and all estimated poses are aligned with the COLMAP(GT). Our poses closely adhere to the ground truth pose, even in sparse view settings with significant motion.}
    \label{fig:main_figure}
\end{figure}

==> figures/results_mip360.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    % \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \tiny

    % \begin{tabular}[b]{cccccccccc}
    \begin{tabular}[b]{ccccccccc}
    
        % \hline
         % Novel View & NeRF & \tiny{Mip-Sp} & Db & DP & BAD & \tiny{ExBluRF} & PDRF & Ours & G.T.\\
         \tiny{Novel View} & \tiny{NeRF} & \tiny{Mip-Sp} & \tiny{Db-NeRF} & \tiny{DP-NeRF} & \tiny{ExBluRF} & \tiny{PDRF} & \tiny{Ours} & \tiny{G.T.}\\
         
        
        % & & 5 hrs & 25 mins & 50 mins & 90 mins & 20 hrs& 80 mins& \\

        \begin{subfigure}[b]{0.19\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurdecoration/004_blurdecoration_gt.png}
            \caption{\tiny{PSNR/SSIM}}
        \end{subfigure} 
        &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurdecoration/004_blurdecoration_nerf_cut.png}
            \caption{\tiny{22.6/.621}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurdecoration/004_blurdecoration_mipsp_cut.png}
            \caption{\tiny{22.5/.658}}
        \end{subfigure} 
        &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurdecoration/004_blurdecoration_deblur_nerf_cut.png}
            \caption{\tiny{25.35/.815}}
        \end{subfigure} 
        &
        \begin{subfigure}[b]{0.097\linewidth} % dp-nerf
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurdecoration/004_blurdecoration_dp_nerf_cut.png}
            \caption{\tiny{{25.54/.826}}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurdecoration/004_blurdecoration_exblurf_cut.png}
            \caption{\tiny{23.39/.761}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurdecoration/004_blurdecoration_pdrf_cut.png}
            \caption{\tiny{24.87/.793}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurdecoration/004_blurdecoration_ours_cut.png}
            \caption{\tiny{\tp{28.74}/\secp{.934}}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurdecoration/004_blurdecoration_gt_cut.png}
            \caption{\tiny{Motion}}
        \end{subfigure}\\ 


        %%%%%%%%% blurgirl
        \begin{subfigure}[b]{0.19\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurgirl/003_blurgirl_gt.png}
            \caption{\tiny{PSNR/SSIM}}
        \end{subfigure} 
        &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurgirl/003_blurgirl_nerf_cut.png}
            \caption{\tiny{23.29/.814}}
        \end{subfigure}&
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurgirl/003_blurgirl_mipsp_cut.png}
            \caption{\tiny{23.27/.845}}
        \end{subfigure} 
        &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurgirl/003_blurgirl_deblur_nerf_cut.png}
            \caption{\tiny{27.08/.902}}
        \end{subfigure} 
        &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurgirl/003_blurgirl_dp_nerf_cut.png}
            \caption{\tiny{{27.54/.908}}}
        \end{subfigure}&
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurgirl/003_blurgirl_exblurf_cut.png}
            \caption{\tiny{25.66/.892}}
        \end{subfigure}&  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurgirl/003_blurgirl_pdrf_cut.png}
            \caption{\tiny{{26.66/.898}}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurgirl/003_blurgirl_ours_cut.png}
            \caption{\tiny{\tp{28.03}/\secp{.927}}}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figs/results_vis/Motion/blurgirl/003_blurgirl_gt_cut.png}
            \caption{\tiny{Motion}}
        \end{subfigure}\\ 
        
        % \hline
    \end{tabular}


    % \setcounter{figure}{4}
    \caption{Visualizations of test views on camera motion and defocus blur dataset. Mip-Sp and Db-NeRF are short for Mip-Splatting \cite{mipsplatting} and Deblur-NeRF \cite{ma2022deblur}.}
    \label{tab:visualization}
    % \vspace{-2em}

\end{figure*}





==> sec/3_method_old.tex <==
\section{SPARS3R}
As show in \cref{fig:pipeline}, SPARS3R builds upon the advancement in MASt3R~\cite{leroy2024grounding} as a pre-trained 3D prior for sparse-view reconstruction. The goal of SPARS3R is to resolve the inaccurate pose estimation from MASt3R and the sparse point cloud from conventional SfM approach.

\input{figures/Poses/pose}
To this end, SPARS3R first performs SfM based on image correspondences, either from MASt3R or other feature matching methods, to obtain a reliable point cloud. This SfM point cloud is then aligned with the dense point cloud produced by MASt3R via local rigid transformations. Specifically, we apply semantic segmentation to partition each image into distinct regions (\cref{semantic_align}), and then apply Procrustes Analysis to estimate rigid transformations per region, yielding a dense SfM-aligned point cloud initialization for the subsequent 3D Gaussian Splatting (\cref{procrustes}).
% Given sparse images, SPARS3R leverages MASt3R \cite{leroy2024grounding} to produce a globally aligned 3D point map. This point map is further aligned with SfM via local rigid transformations informed by semantic heuristics. Specifically, we use a segmentation model to partition each image into distinct regions (\cref{semantic_align}), and then apply Procrustes Analysis to estimate rigid transformations per region, yielding a dense SfM-aligned point cloud initialization for the subsequent 3D Gaussian Splatting (\cref{procrustes}).


% \subsection{Preliminaries}
% \label{3dgs_mast3r}
% Previous work 3DGS \cite{kerbl20233d} proposed to utilize a set of 3D Gaussian primitives \cite{zwicker2001surface} $\{\mathcal{G}_n|n=1,...,N\}$ to represent 3D scenes. Specifically, these 3D Gaussian primitives are parametrized explicitly by a mean $\mathbf{p}_n\in \mathbb{R}^{3 \times 1}$ and a 3D covariance matrix $\Sigma_{n} \in \mathbb{R}^{3 \times 3}$, defining their position, scale, and rotation at a spatial point $\mathbf{x}\in \mathbb{R}^{3 \times 1}$. Concretely,

% \begin{equation}
% % \setlength\abovedisplayskip{5pt}
% % \setlength\belowdisplayskip{5pt}
% \label{Eq:gaussian}
%     \mathcal{G}_n(\mathbf{x}) = e^{-\frac{1}{2}(\mathbf{x}-\mathbf{p}_n)^{T}\Sigma^{-1}_{n}(\mathbf{x}-\mathbf{p}_n)}.
% \end{equation}
% %
% Additionally, each Gaussian also has an opacity $\alpha_n$ and a color $\mathbf{c}_n$. During rendering, we first project the 3D Gaussians to 2D Gaussians using a world-to-camera transformation matrix $W$ and the Jacobian $J$ of the affine approximation of the projective transformation. This projection is noted as follows:

% \begin{equation}
% % \setlength\abovedisplayskip{5pt}
% % \setlength\belowdisplayskip{5pt}
% \label{Eq:gaussian2d}
%     \mathbf{p}^{\textrm{2D}}_n = J W \mathbf{p}_n, \ \  \Sigma^{\textrm{2D}}_n = J W \Sigma_n W^T J^T.
% \end{equation}
% %
% Subsequently, we sort the 2D Gaussians by depth and use volumetric alpha blending to compute the final color for each pixel $x$ as follow:

% \begin{equation}
% \label{gsrender}
% \begin{gathered}
%     \tilde{C}(x)=\sum_{i=1}^{B} {c}_i \alpha_i \mathcal{G}^{\textrm{2D}}_i T_i, \ \ 
%     T_i = \prod_{j=1}^{i-1}(1-\alpha_j\mathcal{G}^{\textrm{2D}}_j),
% \end{gathered}
% \end{equation}
% %
% where $\{1,...,B\}$ denotes the ordered index of Gaussians and $c_i$ is the view-dependent color for the $i$-th Gaussian.

% (maybe also need to cite mast3r+sfm?) 

% DUSt3R \cite{wang2024dust3r} is a 3D foundation model that can generate accurate dense 3D points given an image pair $(n,m)$. DUSt3R outputs pair-wise point maps $X^{n,n},X^{m,n} \in \mathbb{R}^{H \times W \times 3}$, both under image $n$'s coordinate, and their corresponding confidence maps $C^{n}, C^{m} \in \mathbb{R}^{H \times W}$. MASt3R \cite{leroy2024grounding} extends DUSt3R by adding an additional matching head to obtain robust and discriminative local feature descriptors and extract accurate pixel correspondences between images. This auxiliary feature enhances the accuracy of predicting the 3D point maps. 

% When it comes to multiple images, a pairwise view graph $\mathcal{G}(\mathcal{V}, \mathcal{E})$ is constructed where all input images form the vertices $\mathcal{V}$ and visually overlapping images develop edges $\mathcal{E}$, \eg edge $e = (n,m) \in \mathcal{E}$ connecting image $n$ and image $m$.

% post-processing global alignment optimization (Eq. xxx) is performed to align point maps estimated from pair-wise images, resulting in a global-aligned point map.
% \begin{equation}
% \label{gsrender}
% \begin{gathered}
%     \chi^*=\underset{\chi, P, \sigma}{\arg \min } \sum_{e \in \mathcal{E}} \sum_{v \in e} \sum_{i=1}^{H W} C_i^{v, e}\left\|\chi_i^v-\sigma_e P_e X_i^{v, e}\right\|
% \end{gathered}
% \end{equation}
% In our SPARS3R framework, we input the global-aligned point map to the subsequent semantic SfM aligner module.


% Our SPARS3R framework subsequently leverages this globally aligned point map within its Semantic SfM Aligner module for further steps.

% \subsection{Aligning MASt3R with SfM}
\subsection{Enhancing MASt3R with SfM Alignment}
\label{procrustes}
%%% possibly put this in intro
% Why is aligning with SfM important (?): Because MASt3R first generates 3D points and then estimates the camera pose, which could lead to inaccurate pose. In contrast, SfM use a more intricate way to obtain camera poses which are more accurate. As shown in Fig. (put YX's pose figure here), we treat dense SfM as GT and compare the Absolute Trajectory Error (ATE) between SfM and MASt3R. We observe SfM gets more accurate pose.
%%% here just summarize this point
While MASt3R can generate dense 3D points from sparse images, it does not estimate accurate or detailed depth through its pointmap formulation. The regression constraint used in training MASt3R leads to overly smooth results. 
% As illustrated in \cref{fig:depth_comp}, we compare the depths estimated from MASt3R and Marigold \cite{ke2024marigold}, a monocular depth estimator. We observe that MASt3R’s depth map appears notably less smooth and lacks spatial coherence. 
% \input{figures/depth_comp}
\noindent As a result, the camera calibration obtained from such smooth depths is suboptimal and will degrade the fidelity of scene reconstructions. To address this limitation, we propose to align MASt3R's point cloud with that from a conventional SfM pipeline, which provides more accurate camera calibration. We note that, while aligning camera poses from two systems may also be valid, our main goal is to ensure the dense point cloud can be accurately transformed for scene reconstruction.
% which enjoys the best of two worlds by leveraging the strengths of dense point clouds from MASt3R and the precise camera poses provided by SfM. 
This alignment process begins by identifying matching points between the SfM-derived and MASt3R-generated point clouds. Given that MASt3R provides intrinsic pixel-to-3D point correspondences, we can project SfM points onto the image plane, thereby identifying the corresponding points in MASt3R. With these identified correspondences, we apply Procrustes Analysis to estimate a rigid transformation, optimizing for scale, rotation, and translation that minimize the following objective function across the $N_{\textrm{SfM}}$ pairs of matched points. Specifically,
\begin{equation}
\label{Eq:procurstes_align}
\begin{gathered}
    s^*, R^*, t^* = \underset{s, R, t}{\arg \min } \sum_{i=1}^{N_{\textrm{SfM}}} \left\|s R p^{\textrm{M3R}}_i+t-p^{\textrm{SfM}}_i\right\|^2 ,
\end{gathered}
\end{equation}
%
where $\{ (p^{\textrm{M3R}}_i, p^{\textrm{SfM}}_i) | i=1,\cdots, N_{\textrm{SfM}} \}$ denotes $N_{\textrm{SfM}}$ pairs of corresponding MASt3R and SfM points. 
% , and scale $s^*$, rotation $R^*$, and translation $t^*$ are the estimated rigid transformation.
Finally, the estimated rigid transformation is applied to the entire set of $N$ MASt3R points, yielding an accurately aligned dense point cloud: 
%
\begin{equation}
\label{Eq:apply_proc}
\begin{gathered}
    \{ p^{*}_i |  i=1,\cdots,N \},  \ \ 
    p^{*}_i = s^* R^* p^{\textrm{M3R}}_i + t^*.
\end{gathered}
\end{equation}
%
Through this process, the dense point cloud generated by MASt3R gains the added benefit of accurate camera poses from SfM, resulting in a more spatially coherent and geometrically accurate initialization. By integrating precise pose estimations, our approach enhances the structural reliability of the point cloud, improving its suitability for downstream tasks such as 3D scene modeling and reconstruction.


\subsection{Semantic SfM Aligner}
\label{semantic_align}

As discussed in \cref{procrustes}, MASt3R generates noisy and inaccurate depths. This limitation highlights that MASt3R struggles to establish correct depth relationships in complex scenes. For instance, as shown in Fig. xxx, while the depth of individual elements (e.g., the flower and the floor) might be roughly correct, their relative distance do not correlate to their true spatial distance. Relying solely on global alignment under these conditions can lead to dilemmas where only one region aligns correctly. To address this, we propose a semantic heuristic-based approach that segments the scene into localized regions in a cascaded manner, allowing each to be individually aligned as described in \cref{procrustes}. This added flexibility enables more accurate local alignment, significantly improving coherence between MASt3R and SfM depth information.

In more details, we first utilize a segmentation model (SM) to divide each input image, $I_n$, into initial local regions, represented as $\{ \tilde{m}_j \}_{j=1}^{M_1}$, where $\tilde{m}_j$ denotes a binary mask corresponding to the $j$-th region, and $M_1$ is the total number of masks generated by SM. Following this initial segmentation, we further process uncovered areas by reapplying SM to generate additional, finer masks $\{ m'_j \}_{j=1}^{M_2}$, aiming to achieve comprehensive pixel coverage across the image. Specifically,
\begin{equation}
\label{Eq:SAM}
\begin{gathered}
    \{\tilde{m}_j\}_{j=1}^{M_1} = \texttt{SM} (I_n), \ \ 
    \{m'_j\}_{j=1}^{M_2} = \texttt{SM} (I_n \otimes m_0) \\
    m_0 = \neg \left( \cup_{j=1}^{M_1} \tilde{m}_j \right),
    \{ m_j \}_{j=1}^{M} = \{\tilde{m}_j\}_{j=1}^{M_1} \cup \{m'_j\}_{j=1}^{M_2}
\end{gathered}
\end{equation}
% 
where $\otimes$ means element-wise multiplication, and $\neg$ is the logical \texttt{NOT} operator and $m_0$ represents the uncovered area after the initial segmentation. We then get a final distinct, non-overlapping set of masks $\{ m_j \}_{j=1}^{M}$ by combining the masks from two segmentations. Subsequently, we apply the Procrustes Alignment in each masked region $m_j$ following \cref{procrustes} to estimate a rigid transformation that best aligns the local SfM points with their corresponding MASt3R points within that specific mask. Finally, we aggregate these aligned points across all $M$ regions to produce a SfM-aligned dense point cloud, $\{ p_i^* \}_{i=1}^N$, where each point benefits from region-specific adjustments that enhance the overall spatial coherence. Specifically,
\begin{equation}
\label{Eq:semantic_procurstes_align}
\begin{gathered}
    \{s_j^*\}_{j=1}^M, \{R_j^*\}_{j=1}^M, \{t_j^*\}_{j=1}^M = \underset{\{s_j\}, \{R_j\}, \{t_j \} }{\arg \min }
    \sum_{j=1}^{M} \sum_{i=1}^{N_j} \\
    \left\|s_j R_j p^{\textrm{M3R}}_{i,j}+t_j - p^{\textrm{SfM}}_{i,j}\right\|^2 , p^{\textrm{M3R}}_{i,j} \in m_j , \sum_{j=1}^{M}N_j=N_{\textrm{SfM}}. \\
    \{ p_i^* \}_{i=1}^N = \bigcup\limits_{j=1}^M \{ p^{*}_{i,j} \}_j, \ \ 
    p^{*}_{i,j} = s^*_j R^*_j p^{\textrm{M3R}}_{i,j} + t_j^*.
\end{gathered}
\end{equation}
%
% \myparagraph{Discussion} We have also tried panoptic segmentation, \eg ODISE \cite{xu2023odise}. However, it does not work well in our datasets, possibly due to large domain shift. More details can be found in supplementary materials.


\subsection{Optimization}
In addition to the traditional photometric and SSIM loss, we also apply a depth regularization $\mathcal{L}_{\textrm{depth}}$ by maximizing the Pearson correlation between the rendered and monocular depth. Specifically, the final loss is denoted as
\begin{equation}
\label{Eq:training_loss}
\begin{gathered}
    \mathcal{L} = \lambda_1 \| \tilde{C} - C \|_1 + \lambda_2 \textrm{SSIM}(\tilde{C},C) + \lambda_3 \mathcal{L}_{\textrm{depth}} (\tilde{D}, D)
\end{gathered}
\end{equation}
where $\tilde{C}$ and $C$ denote our rendered and Ground Truth RGB image. $\tilde{D}$ and $D$ denote our rendered depth and monocular estimated depth.

During inference, following InstantSplat \cite{fan2024instantsplat}, we also freeze the trained GS model and apply the photometric loss for $500$ iterations to reduce the train-test alignment error because we register train and test views separately and subsequently align them via Procrustes Alignment.

% \left( 1 -\frac{\textrm{Cov}(\tilde{D}, D)}{\sqrt{\textrm{Var}(\tilde{D}) \textrm{Var}(D)}} \right)








==> tables/mips_360.tex <==

% \begin{table*}[!htb]
%     \setlength{\tabcolsep}{2pt}
%     \renewcommand{\arraystretch}{1.11}
%     \centering
%     \small
%     \resizebox{!}{1.8cm}{
%         \begin{tabular}{c | cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
%     \hline
%     \multirow{2}{*}{Methods} &\multicolumn{2}{c|}{Bicycle} & \multicolumn{2}{c|}{Bonsai} & \multicolumn{2}{c|}{Counter} &\multicolumn{2}{c|}{Flowers} & \multicolumn{2}{c|}{Garden} & \multicolumn{2}{c|}{Kitchen} & \multicolumn{2}{c|}{Room} & \multicolumn{2}{c|}{Stump} & \multicolumn{2}{c}{Treehill} & \multicolumn{2}{c}{Average} \\
%     \cline{2-21}
%          & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS  &  PSNR & LPIPS &  PSNR & LPIPS  &  PSNR & LPIPS &  PSNR & LPIPS & \textbf{PSNR} & \textbf{LPIPS}\\
%      \hline
%      3DGS~\cite{kerbl20233d} & 15.17 & 0.535 & 16.99 & 0.359 & 17.12 & 0.340 & 11.96 & 0.607 & 17.17 & 0.349 & 18.83 & 0.265 & 17.94 & 0.346 & 18.25 & 0.435 & 
% 13.74 & 0.607 & 16.35 & 0.427 \\

%      FSGS~\cite{zhu2025fsgs}& 17.14 & 0.685 & 18.39 & 0.364 & 17.41 & 0.409 & 13.39 & 0.802 & 18.99 & 0.454  &  18.16 & 0.287 &  18.31 & 0.345  &  18.86 & 0.745 &  \tp{16.09} & 0.732  & 17.41 & 0.536\\

%      SparseGS~\cite{xiong2023sparsegs}& 16.21 & 0.504 & 16.69 & 0.351 & 17.40 & 0.330 & 12.82 & 0.595 & 17.50 & 0.365  &  18.89 & 0.252 &  17.66 & 0.349  &  18.42 & 0.423 & 14.90 & 0.624 & 16.73 & 0.421\\

%      DNGS~\cite{li2024dngs}& 14.26 & 0.949 & 14.67 & 0.662 & 13.01 & 0.736 & 12.12 & 0.932  & 15.55 & 0.945 & 16.74 & 0.612  &  16.50 & 0.562 & 16.84 & 0.887 & 13.48 & 0.935 & 14.80 & 0.802\\

%       DRGS~\cite{chung2024depth}& 16.24 & 0.750 & 15.71 & 0.589 & 17.33 & 0.520 & 13.18 & 0.889  & 17.49 & 0.624 & 18.18 & 0.482  &  17.67 & 0.442 & 18.24 & 0.702 & 14.45 & 0.800 & 16.50 & 0.644\\

%      CF-3DGS~\cite{Fu_2024_CVPR}& 13.37 & 0.747 & 13.11 & 0.723 & 11.76 & 0.784 & 11.32 & 0.669 & 14.67 & 0.602  &  13.45 & 0.701 &  11.25 & 0.753  &  17.40 & 0.555 &  13.07 & 0.750 & 13.27 & 0.698\\

%      InstantSplat~\cite{fan2024instantsplat}& 15.26 & 0.697 & 15.40 & 0.548 & 16.92 & 0.413 & 13.74 & 0.716 & 17.47 & 0.514  &  18.11 & 0.311 &  18.32 & 0.363  &  16.32 & 0.623 &  15.05 & 0.673 & 17.41 & 0.536\\

%      SPARS3R& \tp{18.42} & \fp{0.362} & \tp{18.68} & \fp{0.326} & \tp{19.64} & \fp{0.273} & \tp{14.67} & \fp{0.472} & \tp{20.25} & \fp{0.235} & \tp{20.72} & \fp{0.183}  &  \tp{20.24} & \fp{0.265} &  \tp{20.18} & \fp{0.369}  &  \tp{16.09} & \fp{0.474}  & \tp{18.77} & \fp{0.329}\\
%     \hline
%     \end{tabular}
%     }
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}





\begin{table*}[!htb]
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.11}
    \centering
    \small
    \resizebox{!}{2cm}{
        \begin{tabular}{c | cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
    \hline
    \multirow{2}{*}{Methods} &\multicolumn{2}{c|}{Bicycle} & \multicolumn{2}{c|}{Bonsai} & \multicolumn{2}{c|}{Counter} &\multicolumn{2}{c|}{Flowers} & \multicolumn{2}{c|}{Garden} & \multicolumn{2}{c|}{Kitchen} & \multicolumn{2}{c|}{Room} & \multicolumn{2}{c|}{Stump} & \multicolumn{2}{c|}{Treehill} & \multicolumn{2}{c}{\textbf{Average}} \\
    \cline{2-21}
         & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS  &  PSNR & LPIPS &  PSNR & LPIPS  &  PSNR & LPIPS &  PSNR & LPIPS & \textbf{PSNR} & \textbf{LPIPS}\\
     \hline
     Instant-NGP~\cite{muller2022instant}& 15.07 & 0.650 & 14.19 & 0.702 & 14.83 & 0.691 & 12.64 & 0.705 & 13.86 & 0.781 & 17.17 & 0.513 & 14.37 & 0.685 & 15.89 & 0.717 & 15.40 & 0.653 & 14.82 & 0.678\\
     3DGS~\cite{kerbl20233d} & 15.17 & 0.535 & 16.99 & 0.359 & 17.12 & 0.340 & 11.96 & 0.607 & 17.17 & 0.349 & 18.83 & 0.265 & 17.94 & 0.346 & 18.25 & 0.435 & 
13.74 & 0.607 & 16.35 & 0.427 \\

     FSGS~\cite{zhu2025fsgs}& 17.14 & 0.685 & 18.39 & 0.364 & 17.41 & 0.409 & 13.39 & 0.802 & 18.99 & 0.454  &  18.16 & 0.287 &  18.31 & 0.345  &  18.86 & 0.745 &  16.09 & 0.732  & 17.41 & 0.536\\

     SparseGS~\cite{xiong2023sparsegs}& 16.21 & 0.504 & 16.69 & 0.351 & 17.40 & 0.330 & 12.82 & 0.595 & 17.50 & 0.365  &  18.89 & 0.252 &  17.66 & 0.349  &  18.42 & 0.423 & 14.90 & 0.624 & 16.73 & 0.421\\

     DNGS~\cite{li2024dngs}& 14.26 & 0.949 & 14.67 & 0.662 & 13.01 & 0.736 & 12.12 & 0.932  & 15.55 & 0.945 & 16.74 & 0.612  &  16.50 & 0.562 & 16.84 & 0.887 & 13.48 & 0.935 & 14.80 & 0.802\\

      DRGS~\cite{chung2024depth}& 16.24 & 0.750 & 15.71 & 0.589 & 17.33 & 0.520 & 13.18 & 0.889  & 17.49 & 0.624 & 18.18 & 0.482  &  17.67 & 0.442 & 18.24 & 0.702 & 14.45 & 0.800 & 16.50 & 0.644\\

     CF-3DGS~\cite{Fu_2024_CVPR}& 13.37 & 0.747 & 13.11 & 0.723 & 11.76 & 0.784 & 11.32 & 0.669 & 14.67 & 0.602  &  13.45 & 0.701 &  11.25 & 0.753  &  17.40 & 0.555 &  13.07 & 0.750 & 13.27 & 0.698\\

     InstantSplat~\cite{fan2024instantsplat}& 15.26 & 0.697 & 15.40 & 0.548 & 16.92 & 0.413 & 13.74 & 0.716 & 17.47 & 0.514  &  18.11 & 0.311 &  18.32 & 0.363  &  16.32 & 0.623 &  15.05 & 0.673 & 17.41 & 0.536\\

     SPARS3R& \tp{18.42} & \fp{0.362} & \tp{19.11} & \fp{0.313} & \tp{19.64} & \fp{0.273} & \tp{14.67} & \fp{0.472} & \tp{20.25} & \fp{0.235} & \tp{20.73} & \fp{0.182} & \tp{20.24} & \fp{0.265} & \tp{20.18} & \fp{0.369} & \tp{16.25} & \fp{0.472}  & \textbf{\tp{19.16}} & \textbf{\fp{0.308}} \\
    \hline
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:my_label}
\end{table*}



==> tables/mv.tex <==

% \begin{table*}[!htb]
%     \setlength{\tabcolsep}{2pt}
%     \renewcommand{\arraystretch}{1.11}
%     \centering
%     \small
%     \resizebox{!}{2.2cm}{
%         \begin{tabular}{c | cc|cc|cc|cc|cc|cc|cc}
%     \toprule
%     \multirow{2}{*}{Methods} &\multicolumn{2}{c|}{Bench} & \multicolumn{2}{c|}{Bicycle} & \multicolumn{2}{c|}{Car} &\multicolumn{2}{c|}{Chair} & \multicolumn{2}{c|}{Ladder} & \multicolumn{2}{c|}{Suv} & \multicolumn{2}{c|}{Table} & \multicolumn{2}{c|}{Average} \\
%     \cline{2-15}
%          & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS  &  PSNR & LPIPS &  PSNR & LPIPS &  PSNR & LPIPS\\
%      \hline
%      3DGS~\cite{kerbl20233d} & 17.19 & 0.184 & 16.28 & 0.200 & 26.58 & 0.092 & 19.85 & 0.260 & 
% 16.64 & 0.226 & 24.91 & 0.072 & 21.55 & 0.193  \\

%      FSGS~\cite{zhu2025fsgs}& 17.59 & 0.176 & 16.71 & 0.199 & 27.53 & 0.085 & 20.45 & 0.275 & 17.89 & 0.268 & 25.78 & 0.072 & 22.61 & 0.238 \\

%      SparseGS~\cite{xiong2023sparsegs}& 17.01 & 0.204 & 16.07 & 0.218 & 27.08 & 0.092 & 19.96 & 0.284 & 17.33 & 0.220 & 25.33 & 0.067 & 21.54 & 0.212  \\

%      DNGS~\cite{li2024dngs}& 17.01 & 0.204 & 16.07 & 0.218 & 27.08 & 0.092 & 19.96 & 0.284 & 
% 17.33 & 0.220 & 25.33 & 0.067 & 21.54 & 0.212  \\

%       DRGS~\cite{chung2024depth}& 17.91 & 0.568 & 17.18 & 0.538 & 23.93 & 0.231 & 20.38 & 0.517 & 
% 14.43 & 0.633 & 24.19 & 0.109 & 21.66 & 0.515  \\

%      CF-3DGS~\cite{Fu_2024_CVPR}& 13.47 & 0.596 & 11.71 & 0.565 & 16.51 & 0.398 & 18.04 & 0.678 & 
% 14.93 & 0.563 & 17.48 & 0.295 & 15.85 & 0.718  \\

%      InstantSplat~\cite{fan2024instantsplat}& 21.14 & 0.315 & 19.67 & 0.355 & 27.28 & 0.133 & 24.59 & 0.262 & 
% 18.55 & 0.359 & 28.01 & 0.074 & 23.30 & 0.238 \\

%      SPARS3R& \tp{25.09} & \fp{0.115} & \tp{23.16} & \fp{0.136} & \tp{29.89} & \fp{0.061} & \tp{28.88} & \fp{0.129} & 
% \tp{19.13} & \fp{0.177} & \tp{29.48} & \fp{0.057} & \tp{24.63} & \fp{0.127} \\
%     \bottomrule
%     \end{tabular}
% }
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}


\begin{table*}[!htb]
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.11}
    \centering
    \small
    \resizebox{!}{2.2cm}{
        \begin{tabular}{c | cc|cc|cc|cc|cc|cc|cc|cc}
    \toprule
    \multirow{2}{*}{Methods} &\multicolumn{2}{c|}{Bench} & \multicolumn{2}{c|}{Bicycle} & \multicolumn{2}{c|}{Car} &\multicolumn{2}{c|}{Chair} & \multicolumn{2}{c|}{Ladder} & \multicolumn{2}{c|}{Suv} & \multicolumn{2}{c|}{Table} & \multicolumn{2}{c}{\textbf{Average}} \\
    \cline{2-17}
         & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS  &  PSNR & LPIPS &  PSNR & LPIPS &  \textbf{PSNR} & \textbf{LPIPS}\\
     \hline
     Instant-NGP~\cite{muller2022instant} & 13.61 & 0.936 & 12.20 & 0.932 & 12.78 & 0.847 & 15.59 & 0.829 & 12.75 & 0.927 & 12.51 & 0.918 & 13.49 & 0.852 & 13.28 & 0.892\\
     3DGS~\cite{kerbl20233d} & 17.19 & 0.184 & 16.28 & 0.200 & 26.58 & 0.092 & 19.85 & 0.260 & 
16.64 & 0.226 & 24.91 & 0.072 & 21.55 & 0.193 & 20.28 & 0.175 \\

     FSGS~\cite{zhu2025fsgs}& 17.59 & 0.176 & 16.71 & 0.199 & 27.53 & 0.085 & 20.45 & 0.275 & 17.89 & 0.268 & 25.78 & 0.072 & 22.61 & 0.238 & 21.08 & 0.188 \\

     SparseGS~\cite{xiong2023sparsegs}& 17.01 & 0.204 & 16.07 & 0.218 & 27.08 & 0.092 & 19.96 & 0.284 & 17.33 & 0.220 & 25.33 & 0.067 & 21.54 & 0.212 & 20.76 & 0.185 \\

     DNGS~\cite{li2024dngs}& 17.01 & 0.204 & 16.07 & 0.218 & 27.08 & 0.092 & 19.96 & 0.284 & 
17.33 & 0.220 & 25.33 & 0.067 & 21.54 & 0.212 & 20.76 & 0.185 \\

      DRGS~\cite{chung2024depth}& 17.91 & 0.568 & 17.18 & 0.538 & 23.93 & 0.231 & 20.38 & 0.517 & 
14.43 & 0.633 & 24.19 & 0.109 & 21.66 & 0.515 & 19.81 & 0.373 \\

     CF-3DGS~\cite{Fu_2024_CVPR}& 13.47 & 0.596 & 11.71 & 0.565 & 16.51 & 0.398 & 18.04 & 0.678 & 
14.93 & 0.563 & 17.48 & 0.295 & 15.85 & 0.718 & 15.43 & 0.545 \\

     InstantSplat~\cite{fan2024instantsplat}& 21.14 & 0.315 & 19.67 & 0.355 & 27.28 & 0.133 & 24.59 & 0.262 & 
18.55 & 0.359 & 28.01 & 0.074 & 23.30 & 0.238 & 23.36 & 0.248 \\

     SPARS3R& \tp{25.09} & \fp{0.115} & \tp{23.16} & \fp{0.136} & \tp{29.89} & \fp{0.061} & \tp{28.88} & \fp{0.129} & \tp{19.13} & \fp{0.177} & \tp{29.48} & \fp{0.057} & \tp{25.31} & \fp{0.122} & \textbf{\tp{25.94}} & \textbf{\fp{0.112}}\\
    \bottomrule
    \end{tabular}
}
    \caption{Performance of various methods on different categories, showing PSNR and LPIPS metrics.}
    \label{tab:my_label}
\end{table*}



==> tables/tanks.tex <==

\begin{table*}[!htb]
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.11}
    \centering
    \small
    \resizebox{!}{2cm}{
        \begin{tabular}{c | cc|cc|cc|cc|cc|cc|cc|cc| cc}
    \hline
    \multirow{2}{*}{Methods} &\multicolumn{2}{c|}{Ballroom} & \multicolumn{2}{c|}{Barn} & \multicolumn{2}{c|}{Church} &\multicolumn{2}{c|}{Family} & \multicolumn{2}{c|}{Francis} & \multicolumn{2}{c|}{Horse} & \multicolumn{2}{c|}{Ignatius} & \multicolumn{2}{c|}{Museum} & \multicolumn{2}{c}{\textbf{Average}}\\
    \cline{2-19}
         & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS & PSNR & LPIPS  &  PSNR & LPIPS &  PSNR & LPIPS  &  PSNR & LPIPS &  \textbf{PSNR} & \textbf{LPIPS} \\
     \hline
     Instant-NGP~\cite{muller2022instant} & 12.05 & 0.464 & 17.97 & 0.233 & 16.64 & 0.317 & 13.72 & 0.359 & 15.05 & 0.583 & 13.39 & 0.538 & 14.46 & 0.440 & 18.97 & 0.183 & 15.28 & 0.389\\
     3DGS~\cite{kerbl20233d} & 15.86 & 0.118 & 20.71 & 0.111 & 17.61 & 0.171 & 20.63 & 0.150 & 
20.59 & 0.229 & 21.38 & 0.150 & 17.68 & 0.151 & 23.75 & 0.056 & 19.78 & 0.142 \\

     FSGS~\cite{zhu2025fsgs}& 15.95 & 0.118 & 21.54 & 0.110 & 18.06 & 0.164 & 24.67 & 0.070 & 22.64 & 0.142  &  27.76 & 0.062 &  17.87 & 0.158  &  24.12 & 0.054 & 21.58 & 0.110\\

     SparseGS~\cite{xiong2023sparsegs}& 15.95 & 0.127 & 20.84 & 0.128 & 17.71 & 0.164 & 21.62 & 0.136 &21.59 & 0.230 & 20.55 & 0.189 & 17.82 & 0.175 & 23.66 & 0.058 & 19.97 & 0.151 \\

     DNGS~\cite{li2024dngs}& 16.10 & 0.271 & 21.32 & 0.355 & 17.46 & 0.422 & 22.11 & 0.256 & 
21.92 & 0.432 & 22.65 & 0.221 & 18.07 & 0.486 & 23.17 & 0.138 & 20.35 & 0.323 \\

      DRGS~\cite{chung2024depth}& 15.96 & 0.211 & 19.16 & 0.281 & 17.62 & 0.335 & 18.99 & 0.307 & 
21.06 & 0.454 & 17.00 & 0.332 & 17.77 & 0.411 & 21.25 & 0.176 & 18.60 & 0.313 \\

     CF-3DGS~\cite{Fu_2024_CVPR}& 23.19 & 0.102 & 17.38 & 0.375 & 18.96 & 0.286 & 17.63 & 0.301 & 
19.99 & 0.357 & 17.22 & 0.361 & 21.10 & 0.174 & 16.46 & 0.413 & 18.99 & 0.396 \\

     InstantSplat~\cite{fan2024instantsplat}& 27.78 & 0.069 & 27.37 & 0.116 & 22.91 & 0.168 & 28.29 & 0.087 & 
30.66 & 0.138 & 27.74 & 0.093 & 24.35 & 0.182 & 26.62 & 0.068 & 26.97 & 0.115\\

     SPARS3R& \tp{29.49} & \fp{0.026} & \tp{30.30} & \fp{0.042} & \tp{25.02} & \fp{0.095} & \tp{30.77} & \fp{0.032} & \tp{30.89} & \fp{0.072} & \tp{31.38} & \fp{0.037} & \tp{30.65} & \fp{0.044} & \tp{30.73} & \fp{0.026} & \textbf{\tp{29.90}} & \textbf{\fp{0.047}}\\
    \hline
    \end{tabular}
    }
    \caption{Caption}
    \label{tab:my_label}
\end{table*}



